Skein and cluster algebras with coefficients for unpunctured surfaces

We propose a skein model for the quantum cluster algebras of surface type with coefficients. We introduce a skein algebra $\mathscr{S}_{\Sigma,\mathbb{W}}^{A}$ of a walled surface $(\Sigma,\mathbb{W})$, and prove that it has a quantum cluster structure. The walled surfaces naturally generalize the marked surfaces with multi-laminations, which have been used to describe the quantum cluster algebras of geometric type for marked surfaces by Fomin--Thurston [FT18]. Moreover, we give skein theoretic interpretation for some of quasi-homomorphisms [Fra16] between these quantum cluster algebras.

==> figure/tikz_reduction.tex <==
\begin{align*}
    S_1&\colon
    \ \tikz[baseline=-.6ex, scale=.1]{
        \draw[webline] (-45:5) -- (135:5);
        \draw[webline, overarc] (-135:5) -- (45:5);
    }\ 
    \leadsto
    A
    \ \tikz[baseline=-.6ex, scale=.1]{
        \draw[webline] (45:5) to[out=south west, in=north west] (-45:5);
        \draw[webline] (-135:5) to[out=north east, in=south east] (135:5);
    }\ 
    +A^{-1}
    \ \tikz[baseline=-.6ex, scale=.1]{
        \draw[webline] (-45:5) to[out=north west, in=north east] (-135:5);
        \draw[webline] (135:5) to[out=south east, in=south west] (45:5);
    }\ ,&
    S_2&\colon
    \ \tikz[baseline=-.6ex, scale=.1]{
        \draw[webline] (0,0) circle [radius=4cm];
    }\ 
    \leadsto
    (-A^2-A^{-2})\ \textcolor{red}{\emptyset},\\
    S_3&\colon
    \ \tikz[baseline=-.6ex, scale=.1, yshift=-2cm]{
        \coordinate (A) at (-6,0);
        \coordinate (B) at (6,0);
        \coordinate (P) at (0,0);
        \draw[webline, shorten <=.2cm] (P) -- (110:6);
        \draw[webline] (P) -- (70:6);
        \draw[dashed] (30:6) arc (30:150:6cm);
        \draw[dashed] (P) -- (30:6);
        \draw[dashed] (P) -- (150:6);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
    }\ 
    \leadsto A^{\frac{1}{2}}
    \ \tikz[baseline=-.6ex, scale=.1, yshift=-2cm]{
        \coordinate (A) at (-6,0);
        \coordinate (B) at (6,0);
        \coordinate (P) at (0,0);
        \draw[webline] (P) -- (110:6);
        \draw[webline] (P) -- (70:6);
        \draw[dashed] (30:6) arc (30:150:6cm);
        \draw[dashed] (P) -- (30:6);
        \draw[dashed] (P) -- (150:6);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
    }\ ,& 
    &\ \tikz[baseline=-.6ex, scale=.1, yshift=-2cm]{
        \coordinate (A) at (-6,0);
        \coordinate (B) at (6,0);
        \coordinate (P) at (0,0);
        \draw[webline] (P) -- (110:6);
        \draw[webline, shorten <=.2cm] (P) -- (70:6);
        \draw[dashed] (30:6) arc (30:150:6cm);
        \draw[dashed] (P) -- (30:6);
        \draw[dashed] (P) -- (150:6);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
    }\ 
    \leadsto A^{-\frac{1}{2}}    
    \ \tikz[baseline=-.6ex, scale=.1, yshift=-2cm]{
        \coordinate (A) at (-6,0);
        \coordinate (B) at (6,0);
        \coordinate (P) at (0,0);
        \draw[webline] (P) -- (110:6);
        \draw[webline] (P) -- (70:6);
        \draw[dashed] (30:6) arc (30:150:6cm);
        \draw[dashed] (P) -- (30:6);
        \draw[dashed] (P) -- (150:6);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
    }\ ,\\
    S_4&\colon
    \ \tikz[baseline=-.6ex, scale=.1, yshift=-2cm]{
        \coordinate (A) at (-6,0);
        \coordinate (B) at (6,0);
        \coordinate (P) at (0,0);
        \draw[webline, rounded corners] (P) -- (110:4) -- (70:4) -- (P);
        \draw[dashed] (30:6) arc (30:150:6cm);
        \draw[dashed] (P) -- (30:6);
        \draw[dashed] (P) -- (150:6);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
    }\ 
    \leadsto 0, &
    S_5&\colon
    \ \tikz[baseline=-.6ex, scale=.08, yshift=-5cm]{
        \draw[webline, rounded corners] (-5,0) -- (5,5) -- (-5,10);
        \draw[wline] (0,-1) -- (0,11);
        \node at (0,11) [below right]{\scriptsize $\nu$};
    }\ 
    \leadsto a_\nu
    \ \tikz[baseline=-.6ex, scale=.08, yshift=-5cm]{
            \draw[webline, rounded corners] (-5,0) -- (-2,5) -- (-5,10);
            \draw[wline] (0,-1) -- (0,11);
            \node at (0,11) [below right]{\scriptsize $\nu$};
    }\ ,\\
    S_6&\colon
    \ \tikz[baseline=-.6ex, scale=.08, yshift=-2cm]{
        \coordinate (A) at (-10,0);
        \coordinate (B) at (10,0);
        \coordinate (P) at (0,0);
        \draw[webline, rounded corners] (P) -- (60:6) -- (120:10);
        \draw[wline] (P) -- (90:10);
        \draw[dashed] (30:10) arc (30:150:10cm);
        \draw[dashed] (P) -- (30:10);
        \draw[dashed] (P) -- (150:10);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
        \node at (90:10) [below right]{\scriptsize $\nu$};
    }\ 
    \leadsto z_{\nu,+}
    \ \tikz[baseline=-.6ex, scale=.08, yshift=-2cm]{
        \coordinate (A) at (-10,0);
        \coordinate (B) at (10,0);
        \coordinate (P) at (0,0);
        \draw[webline, rounded corners] (P) -- (120:10);
        \draw[wline] (P) -- (90:10);
        \draw[dashed] (30:10) arc (30:150:10cm);
        \draw[dashed] (P) -- (30:10);
        \draw[dashed] (P) -- (150:10);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
        \node at (90:10) [below right]{\scriptsize $\nu$};
    }\ ,&
    S_7&\colon
    \ \tikz[baseline=-.6ex, scale=.08, yshift=-2cm]{
        \coordinate (A) at (-10,0);
        \coordinate (B) at (10,0);
        \coordinate (P) at (0,0);
        \draw[webline, rounded corners] (P) -- (120:6) -- (60:10);
        \draw[wline] (P) -- (90:10);
        \draw[dashed] (30:10) arc (30:150:10cm);
        \draw[dashed] (P) -- (30:10);
        \draw[dashed] (P) -- (150:10);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
        \node at (90:10) [below left]{\scriptsize $\nu$};
    }\ 
    \leadsto z_{\nu,-}
    \ \tikz[baseline=-.6ex, scale=.08, yshift=-2cm]{
        \coordinate (A) at (-10,0);
        \coordinate (B) at (10,0);
        \coordinate (P) at (0,0);
        \draw[webline, rounded corners] (P) -- (60:10);
        \draw[wline] (P) -- (90:10);
        \draw[dashed] (30:10) arc (30:150:10cm);
        \draw[dashed] (P) -- (30:10);
        \draw[dashed] (P) -- (150:10);
        \bdryline{(A)}{(B)}{2cm}
        \draw[fill=black] (P) circle [radius=20pt];
        \node at (90:10) [below left]{\scriptsize $\nu$};
    }\ ,
\end{align*}

